The Isomorphism Problem of Power Graphs and a Question of Cameron

The isomorphism problem for graphs (GI) and the isomorphism problem for groups (GrISO) have been studied extensively by researchers. The current best algorithms for both these problems run in quasipolynomial time. In this paper, we study the isomorphism problem of graphs that are defined in terms of groups, namely power graphs, directed power graphs, and enhanced power graphs. It is not enough to check the isomorphism of the underlying groups to solve the isomorphism problem of such graphs as the power graphs (or the directed power graphs or the enhanced power graphs) of two nonisomorphic groups can be isomorphic. Nevertheless, it is interesting to ask if the underlying group structure can be exploited to design better isomorphism algorithms for these graphs. We design polynomial time algorithms for the isomorphism problems for the power graphs, the directed power graphs and the enhanced power graphs arising from finite nilpotent groups. In contrast, no polynomial time algorithm is known for the group isomorphism problem, even for nilpotent groups of class 2. We note that our algorithm does not require the underlying groups of the input graphs to be given. The isomorphism problems of power graphs and enhanced power graphs are solved by first computing the directed power graphs from the input graphs. The problem of efficiently computing the directed power graph from the power graph or the enhanced power graph is due to Cameron [IJGT'22]. Therefore, we give a solution to Cameron's question.

==> citation.tex <==
% \textbf{Papers related to group isomorphism}

% Algorithms for group isomorphism via group extensions and cohomology \cite{grochow2017algorithms}

% On p-Group Isomorphism: Search-To-Decision,
% Counting-To-Decision, and Nilpotency Class
% Reductions via Tensors \cite{grochow2021p}

% Efficient isomorphism testing for a class of group extensions \cite{gall2008efficient}

% On the $n^{\log n}$ isomorphism technique (a preliminary report) \cite{miller1978nlog}

% On isomorphism testing of groups with normal Hall subgroups \cite{qiao2012isomorphism}

% Bidirectional collision detection and faster deterministic isomorphism testing \cite{rosenbaum2013bidirectional}

% Breaking the $n^{\log n}$ Barrier for Solvable-Group Isomorphism \cite{rosenbaum2013breaking}

% \textbf{Papers related to graph isomorphism}

% Babai graph isomorphism \cite{babai2016graph}

% Luks bounded degree graph isomorphism \cite{luks1982isomorphism}

% Bounded degree Grohe \cite{grohe2020graph}

% k-dimensional WL for treewidth k \cite{kiefer2022power}

% Treewidth Bodlander \cite{bodlaender1990polynomial}

% FPT isomorphism for bounded tree width \cite{lokshtanov2017fixed}

% FPT improved for bounded treewidth graph \cite{grohe2020improved}

% Bounded Rankwidth graph isomorphism \cite{grohe2021isomorphism}

% Rankwidth and clique width relation \cite{oum2006approximating}


% \begin{claim}
% $f_j: V(X_j)\rightarrow V(R_3(j)) $ is well defined, $\forall 1\leq j \leq m$.
% \end{claim}
% \begin{proof}
% Proof is by induction on $m$, the size of a CCG-set of $G$. Our induction hypothesis is $f_j$ is well defined. In base case, Consider $f_1:V(X_1)\xrightarrow{}R_3(1)$. In $R_3(1)=HD[col(g_1)]$, color of every vertex is distinct. So, $x=y\iff col(x)=col(y)$. Consider $x_1$ and $x_2$. If $x_1=x_2$ then $col(x_1)=col(x_2)$. By definition of $f$, $col(x_1)=col(f_1(x_1)$ and $col(x_2)=col(f_1(x_2)$. So, $col(f_1(x_1))=col(f_1(x_2) \implies f_1(x_1)=f_1(x_2)$. So, $f_1$ is well-defined. By induction hypothesis, assume that $f_{j-1}$ is well-defined. Now, for inductive case, consider $f_j:V(X_j)\xrightarrow{} V(R_3(j))$. Consider $x_1=x_2$. If $x_1\in V(X_{j-1})$, then from definition of $f_j$ we have $f_j(x_1)=f_{j-1}(x_1)=f_{j-1}(x_2)=f_j(x_2)$.

% Now, consider the case when $x_1\notin V(X_{j-1}$ then $x_1\in V(X_j)\setminus V(X_{j-1}$. So, $f_j(x_1),f_j(x_2)\in V(R_3(j))\setminus V(R_3(j-1))$. $f_j(x_1),f_j(x_2)\in Des(g_j)$ in $R_3(G)$. 

% $x_1=x_2\iff col(x_1)=col(x_2)\iff col(f_j(x_1))=col(f_j(x_2))\iff f_j(x_1)=f_j(x_2)$. So, $f_j$ is well-defined.
% \end{proof}

% %\section{edge preserving}
% Note that $\{y,y'\}\in E(R_j)$ if and only if (1) $y$,$y' \in Des(g_i)$ for some $1\leq i\leq j$ and (2) $col(y)=p\cdot col(y')$ or $col(y')=p\cdot col(y)$ for some prime $p$.

%     Now, we will show that $f_j$ preserves edge relation between $X_{j}$ and $R_3(j)$. The edges of $X_j$ will fall into one of the cases, not necessarily disjoint.
%     % i.e., $\{x,x'\} \in E(X_j) \ \iff \ \{f(x),f(x')\} \in E(R_3(j))$.
    

% (a) Let $x, x' \in V(X_{j-1})$ (old graph). Then, by definition of $f_j$ in Equation \ref{defintion of f_j}, $f_j(x)=f_{j-1}(x)$ and $f_j(x')=f_{j-1}(x')$. Since by induction hypothesis $f_{j-1}$ is an isomorphism between $X_{j-1}$ and $R_3(j-1)$, so
% % $\{f_j(x),f_j(x')\} \in E(R_3(j-1)) \subseteq E(R_3(j))$,
% $\{x,x'\} \in E(X_{j-1})\subseteq E(X_j) \ \iff \{f(x),f(x')\} \in E(R_3(j-1)) \subseteq E(R_3(j)).$ However, the following may also happen that $\{x,x'\}\notin E(X_{j-1})$ but $\{x,x'\}\in E(X_{j})$. This happens when $x,x'\in X_{j-1,j-1}$ i.e., $x$ is identified with some $y\in Y_{j,j-1}$ and $x'$ is identified with some $y'\in Y_{j,j-1}$ such that $\{x',y'\}\in E(Y_j)$. Similarly, $f_j(x),f_j(x')\in R_3(j-1)$ such that $\{f_j(x),f_j(x')\}\notin E(R_3(j-1))$ but $\{f_j(x),f_j(x')\}\in E(R_3(j))$. This happens only because $f_j(x),f_j(x')\in Des(g_j)\in R_3(j)$ and  $f_j(x),f_j(x')\notin Des(g_i) \forall i\leq j$. In this case, we can see that $\{x,x'\}\in E(X_j)\iff \{f_j(x),f_j(x')\}\in E(R_3(j)$.

% (**Complicated case description, overlapping cases **  )
% (b)  Let $x,x' \in S_1 \sqcup S_2$ where $S_1$ is $V(X_j)\setminus V(X_{j-1}$ and $S_2$ is the set of vertices that are the result of identification of $X_{j-1,j-1}$ and $Y_{j,j-1}$ in the $j^{th}$ iteration. Note that $S_1$ and $S_2$ are disjoint sets. Without loss of generality, we can assume this set as $X_{j-1,j-1}$. It is not hard to see $S_1\sqcup$ corresponds to $V(Y_j)$. Since $Y_j=HD[col(g_j)]\cong R_3(G)[Des(g_j)]$ by \Cref{Des(g_i)=HD[g_i]}, so $\{x,x'\}\in E(X_j)\iff \{f_j(x),f_j(x')\}\in E(R_3(j)$.

% (c) Let $x$ be a vertex from old graphs $X_{j-1}$ which has not been identified in $j^{th}$ iteration i.e., $x \in V(X_{j-1}) \setminus X_{j-1,j-1}$. Let $x'$ be a newly added vertex which has not been identified in $j^{th}$ iteration i.e., $x' \in V(X_j)\setminus V(X_{j-1}).$ It is not hard to see that $\{x,x'\}\notin E(X_{j-1}\sqcup Y_j)$ before the identification process, and so $\{x,x'\}\notin E(X_j)$. Now, $f_j(x) \in V(R_3(j-1))\setminus Des(g_j)$ and $f_j(x') \in V(R_3(j))\setminus V(R_3(j-1)).$ Since, $f_j(x)$ and $f_j(x')$ are not in same $Des(u)$ for any vertex $u$ in $R_3(j)$, therefore $\{f_j(x),f_j(x')\}$ is not an edge in $R_3(j)$. Thus, it is proved that $f_j$ is an isomorphism between $X_j$ and $R_3(j)$. So, we can conclude that $X_m \cong R_3(m).$ It is easy to see that $R_3(m)$ is $R_3(G)$.

\newpage
However, when $x,x'\in X_{j-1,j-1}$, it may happen that $\{x,x'\}\notin E(X_{j-1})$ but $\{x,x'\}\in E(X_j)$. This happens only when $x$ is identified with some $y\in Y_j$ and $x'$ is identified with some $y'\in Y_j$such that $\{y,y'\}\in E(Y_j)$. The latter implies that $col(y)=col(y')\cdot p$ or $col(y')=col(y)\cdot p$ for some prime $p$. Since $\{x,x'\}\notin E(X_{j-1})$, so $\{f_j(x),f_j(x')\}\notin E(R_3(j-1))$. Note that $f_j$ preserves color of the vertices so $f_j(x),f_j(x')\notin Des(g_i) \forall i<j$. Since, $x,x'\in X_{j-1,j-1}$ so $f_j(x),f_j(x')\in Des(g_j)$. 
